Discovering Reliable Causal Rules

We study the problem of deriving policies, or rules, that when enacted on a complex system, cause a desired outcome. Absent the ability to perform controlled experiments, such rules have to be inferred from past observations of the system's behaviour. This is a challenging problem for two reasons: First, observational effects are often unrepresentative of the underlying causal effect because they are skewed by the presence of confounding factors. Second, naive empirical estimations of a rule's effect have a high variance, and, hence, their maximisation can lead to random results. To address these issues, first we measure the causal effect of a rule from observational data---adjusting for the effect of potential confounders. Importantly, we provide a graphical criteria under which causal rule discovery is possible. Moreover, to discover reliable causal rules from a sample, we propose a conservative and consistent estimator of the causal effect, and derive an efficient and exact algorithm that maximises the estimator. On synthetic data, the proposed estimator converges faster to the ground truth than the naive estimator and recovers relevant causal rules even at small sample sizes. Extensive experiments on a variety of real-world datasets show that the proposed algorithm is efficient and discovers meaningful rules.

==> preamble.tex <==
% Show the referenced equations only 
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}

% proof is in the appendix 
\newcommand{\proofApx}{
	\begin{proof}
		We postpone the proof to the Appendix.
	\end{proof}
}

% change the footnote marks
\makeatletter
\renewcommand*{\@fnsymbol}[1]{\ensuremath{\ifcase#1\or   *\or \circ \or \bullet \or \ddagger\or
		\mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger
		\or \ddagger\ddagger \else\@ctrerr\fi}}
\makeatother

% wrap theorem titles
\makeatletter
\renewcommand*{\@opargbegintheorem}[3]{\trivlist
	\item[\hskip \labelsep{\bfseries #1\ #2}] \textsc{(#3)}\ \itshape}
\makeatother

% SVJOUR fixes
%\renewcommand{\email}[1]{\texttt{#1}}

% for math columns in tables
\RequirePackage{array}   		% for \newcolumntype macro
\newcolumntype{L}{>{$}l<{$}} 	% math-mode version of "l" column type
\newcolumntype{R}{>{$}r<{$}} 	% math-mode version of "r" column type
\newcolumntype{C}{>{$}c<{$}} 	% math-mode version of "c" column type

% other effect measures
\newcommand{\wracc}{\ensuremath{\bm{w}(\drule)}\xspace}
\newcommand{\ewracc}{\ensuremath{\widehat{\bm{w}}(\drule)}\xspace}

% project details
\RequirePackage{url}
\newcommand{\codelink}{https://www.dropbox.com/s/frlv8os29gobcby/rce.zip?dl=0\xspace}
\newcommand{\realkd}{realKD\xspace}
\newcommand{\realkdlink}{\url{https://bitbucket.org/realKD/}\xspace}

% color scheme for gray-scale printing
\definecolor{c1}{RGB}{63,87,101}
\definecolor{c2}{RGB}{119,196,211}
\definecolor{c3}{RGB}{255,83,13}
\definecolor{c4}{rgb}{0.21, 0.3, 0.3}

\definecolor{ca}{RGB}{128,128,128}
\definecolor{cb}{RGB}{159,159,159}
\definecolor{cc}{RGB}{253,140,46}
\definecolor{cd}{RGB}{253,253,249}

\definecolor{v1}{RGB}{127,37,251}
\definecolor{v2}{RGB}{252,13,27}
\definecolor{v3}{RGB}{31,182,234}
\definecolor{v4}{RGB}{133,254,182}
\definecolor{v5}{RGB}{253,178,103}

\definecolor{proseco1}{RGB}{40,170,213}
\definecolor{proseco2}{RGB}{178,77,148}
\definecolor{proseco3}{RGB}{56,174,151}
\definecolor{proseco1light}{RGB}{169,221,238}
\definecolor{proseco2light}{RGB}{224,183,212}
\definecolor{proseco3light}{RGB}{175,222,213}

% math notations
\newcommand{\by}[2]{\ensuremath{#1 \times #2}\xspace}
\newcommand{\argmin}{\ensuremath{\operatorname*{argmin}}\xspace}
\newcommand{\argmax}{\ensuremath{\operatorname*{argmax}}\xspace}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\newcommand{\bigmid}{\ensuremath{\,\middle\vert\,}\xspace}
\newcommand{\XX}{% Space between XX varies depending on where it's used
	\mathchoice% https://tex.stackexchange.com/q/148740/5764
	{X\mskip-12.5mu X}% \displaystyle
	{X\mskip-12.5mu X}% \textstyle
	{X\mskip-12mu X}% \scriptstyle
	{X\mskip-11.5mu X}% \scriptscriptstyle
}

% rule notations
\newcommand{\doo}{\ensuremath{\mathit{do}}\xspace}
\newcommand{\union}{\ensuremath{\cup}\xspace}
\newcommand{\intersection}{\ensuremath{\cap}\xspace}
\newcommand{\true}{\ensuremath{ {\scriptstyle \top} }\xspace}
\newcommand{\false}{\ensuremath{ {\scriptstyle \bot} }\xspace}
\newcommand{\target}{\ensuremath{Y}\xspace}
\newcommand{\targetval}{\ensuremath{y}\xspace}
\newcommand{\targetspace}{\ensuremath{\mathcal{Y}}\xspace}

\newcommand{\props}{\ensuremath{\pi}\xspace}
\newcommand{\setofprops}{\ensuremath{\bm{\pi}}\xspace}
\newcommand{\logicaltest}{\ensuremath{\pi}\xspace}
\newcommand{\rulecondition}{\ensuremath{\sigma}\xspace}
\newcommand{\descriptionVars}{\ensuremath{\pmb{\mathbb{X}}}\xspace}

\DeclareFontEncoding{LS1}{}{}
\DeclareFontSubstitution{LS1}{stix}{m}{n}
\DeclareMathAlphabet{\mathscr}{LS1}{stixscr}{m}{n}
\SetMathAlphabet{\mathscr}{bold}{LS1}{stixscr}{b}{n}
\newcommand{\descriptionVarsSpace}{\ensuremath{\bm{\mathscr{X}}}\xspace}

\newcommand{\actionables}{\ensuremath{\pmb{\mathbb{X}}}\xspace}
\newcommand{\actionablesVal}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\actionablesSpace}{\ensuremath{\bm{\mathscr{X}}}\xspace}
\newcommand{\actionable}{\ensuremath{X}\xspace}
\newcommand{\actionableSpace}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\actionablesSubset}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\actionablesSubsetSpace}{\ensuremath{\bm{\mathcal{X}}}\xspace}

\newcommand{\domain}{\ensuremath{\mathrm{dom}}\xspace}
\newcommand{\unit}{\ensuremath{u}\xspace}
\newcommand{\entity}{\ensuremath{e}\xspace}
%\newcommand{\attributes}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\covariates}{\ensuremath{\bm{C}}\xspace}
\newcommand{\attribute}{\ensuremath{X}\xspace}
\newcommand{\attributes}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\attributesval}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\attributesspace}{\ensuremath{\bm{\mathcal{X}}}\xspace}
\newcommand{\attributespace}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\attributesrule}{\ensuremath{\attributes_{\drule}}\xspace}
\newcommand{\attributesrulespace}{\ensuremath{\attributesspace_{\!\drule}}\xspace}
\newcommand{\attributesrulevec}{\ensuremath{\mathbf{x}}\xspace}

%\newcommand{\attribute}{\ensuremath{X}\xspace}
%\newcommand{\control}{\ensuremath{Z}\xspace}
\newcommand{\cov}{\ensuremath{z}\xspace}
\newcommand{\covs}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\covspace}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\control}{\ensuremath{Z}\xspace}
\newcommand{\somecontrols}{\ensuremath{\bm{Z}}\xspace}
\newcommand{\controls}{\ensuremath{\pmb{\mathbb{Z}}}\xspace}
%\newcommand{\controls}{\ensuremath{\mathbf{Z}}\xspace}
\newcommand{\controlsval}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\controlsvec}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\controlvec}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\controlsspace}{\ensuremath{\bm{\mathscr{\control}}}\xspace}
\newcommand{\controlspace}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\latent}{\ensuremath{U}\xspace}
\newcommand{\latents}{\ensuremath{\bm{U}}\xspace}

\newcommand{\controlcol}{\ensuremath{\control^{(\texttt{l})}}\xspace}

\newcommand{\model}{\ensuremath{G}\xspace}

\newcommand{\parents}{\ensuremath{\text{pa}}\xspace}

\newcommand{\drule}{\ensuremath{\sigma}\xspace}
\newcommand{\druleval}{\ensuremath{s}\xspace}
\newcommand{\drulespace}{\ensuremath{\mathcal{L}}\xspace}

\newcommand{\esymb}{\ensuremath{\bm{e}}\xspace}
\newcommand{\ronlysymb}{\ensuremath{\bm{r}}\xspace}
\newcommand{\rsymb}{\ensuremath{\widehat{\ronlysymb}}\xspace}
\newcommand{\eesymb}{\ensuremath{\widehat{\esymb}}\xspace}

\newcommand{\e}{\ensuremath{\esymb(\drule)}\xspace}
%\newcommand{\ec}{\ensuremath{\overrightarrow{\esymb}(\drule)}\xspace}
\newcommand{\ec}{\ensuremath{\esymb(\drule)}\xspace}
\newcommand{\ee}{\ensuremath{\eesymb(\drule)}\xspace}
\newcommand{\ce}{\ensuremath{\esymb(\drule \mid \controls)}\xspace}
\newcommand{\re}{\ensuremath{\rsymb(\drule)}\xspace}
\newcommand{\ece}{\ensuremath{\eesymb(\drule \mid \controls)}\xspace}
\newcommand{\rce}{\ensuremath{\rsymb(\drule \mid \controls)}\xspace}

\newcommand{\az}{\ensuremath{a_z}\xspace}
\newcommand{\bz}{\ensuremath{b_z}\xspace}
\newcommand{\cz}{\ensuremath{c_z}\xspace}
\newcommand{\dz}{\ensuremath{d_z}\xspace}
\newcommand{\nz}{\ensuremath{n_z}\xspace}

\newcommand{\universe}{\ensuremath{U}\xspace}
\newcommand{\sample}{\ensuremath{S}\xspace}
\newcommand{\samplesize}{\ensuremath{N}\xspace}

\newcommand{\ext}{\ensuremath{\bm{\mathrm{ext}}}\xspace}
%\newcommand{\cov}{\ensuremath{\mathbf{cov}}\xspace}
\newcommand{\supp}{\ensuremath{\mathbf{cnt}}\xspace}
%\newcommand{\n}{\ensuremath{n}\xspace}
\newcommand{\N}{\ensuremath{N}\xspace}

\newcommand{\na}{\ensuremath{a}\xspace}
\newcommand{\nb}{\ensuremath{b}\xspace}
\newcommand{\nc}{\ensuremath{c}\xspace}
\newcommand{\nd}{\ensuremath{d}\xspace}

\newcommand{\nap}{\ensuremath{\na'}\xspace}
\newcommand{\nbp}{\ensuremath{\nb'}\xspace}
\newcommand{\ncp}{\ensuremath{\nc'}\xspace}
\newcommand{\ndp}{\ensuremath{\na'}\xspace}

\newcommand{\countconfig}{\ensuremath{\mathcal{C}}\xspace}

\newcommand{\nyone}{\ensuremath{n_1}\xspace}
\newcommand{\nyzero}{\ensuremath{n_0}\xspace}

\newcommand{\nyonez}{\ensuremath{n^1_z}\xspace}
\newcommand{\nyzeroz}{\ensuremath{n^0_z}\xspace}
\newcommand{\none}{\ensuremath{n_1}\xspace}
\newcommand{\nzero}{\ensuremath{n_0}\xspace}

\newcommand{\tloose}{\ensuremath{\bound{\tau}_l}\xspace}
\newcommand{\ttight}{\ensuremath{\bound{\tau}_t}\xspace}
\newcommand{\nloose}{\ensuremath{n_l}\xspace}
\newcommand{\ntight}{\ensuremath{n_t}\xspace}

% math notations
\newcommand{\bound}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\andl}{\ensuremath{\wedge}\xspace}	% logical and
%\newcommand{\expectation}[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}\xspace}
\newcommand{\eexpectationd}{\ensuremath{\hat{\mathbb{E}}}}
\newcommand{\eexpectation}[1]{\ensuremath{\eexpectationd\left[#1\right]}\xspace}
\newcommand{\ezexpectation}[1]{\ensuremath{\eexpectationd\left[#1\right]}\xspace}
\newcommand{\expectation}[1]{\ensuremath{\mathbb{E}\left[#1\right]}\xspace}
\newcommand{\texpectation}[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}\xspace}
\newcommand{\zexpectation}[1]{\ensuremath{\mathbb{E}\left[#1\right]}\xspace}

\newcommand{\mse}{\ensuremath{\operatorname*{MSE}}\xspace}
\newcommand{\n}{\ensuremath{n}\xspace}
\newcommand{\diffsymb}{\ensuremath{\tau}\xspace}
\newcommand{\diff}{\ensuremath{\diffsymb(\controlsval)}\xspace}
\newcommand{\oestdiff}{\ensuremath{\bound{\diffsymb}(\controlsval)}\xspace}
\newcommand{\oestrace}{\ensuremath{\bound{\ronlysymb}}\xspace}

\newcommand{\maxconfint}{\ensuremath{\epsilon}\xspace}
\newcommand{\hatp}{\ensuremath{\hat{p}_{\drule,\controlsval}}\xspace}
\newcommand{\nhatp}{\ensuremath{n_{\drule,\controlsval}}\xspace}
\newcommand{\hatq}{\ensuremath{\hat{p}_{\bar{\drule},\controlsval}}\xspace}
\newcommand{\nhatq}{\ensuremath{n_{\bar{\drule},\controlsval}}\xspace}
\newcommand{\hatPr}{\ensuremath{\hat{\Pr}}\xspace}
\newcommand{\powset}[1]{\ensuremath{\mathcal{P}(#1)}\xspace}
\newcommand{\predicate}{\ensuremath{\pi}\xspace}
\newcommand{\predicatepool}{\ensuremath{\Pi}\xspace}
\newcommand{\searchspace}{\ensuremath{\Omega}\xspace}
\newcommand{\refineop}{\ensuremath{\bm{b}}\xspace}
\newcommand{\func}{\ensuremath{f}\xspace}
\newcommand{\support}{\ensuremath{\mathbf{count}}\xspace}
\newcommand{\coverage}{\ensuremath{\bm{\mathrm{cvg}}}\xspace}
%\newcommand{\conflevel}{\ensuremath{c}\xspace}
\newcommand{\erate}{\ensuremath{\alpha}\xspace}
\newcommand{\zscore}{\ensuremath{\beta}\xspace}
\renewcommand{\Pr}{\ensuremath{P}\xspace}
\newcommand{\pmf}{\ensuremath{p}\xspace}
\newcommand{\empPmf}{\ensuremath{\hat{p}}\xspace}
\newcommand{\policy}{\ensuremath{Q}\xspace}
\newcommand{\topkselectors}{\ensuremath{\mathcal{F}_k}\xspace}
\newcommand{\topkrules}{\ensuremath{\mathcal{F}_k}\xspace}
\newcommand{\dataset}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\indep}{\ensuremath{\perp \! \! \! \perp}\xspace}
\newcommand{\dep}{\centernot{\indep}\xspace}
\newcommand{\lambdaz}{\ensuremath{\lambda_z}\xspace}
\newcommand{\gammaz}{\ensuremath{\gamma_z}\xspace}

% tcs notations
\newcommand{\bigo}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\approxfactor}{\ensuremath{\gamma}\xspace}

% other notations
%\RequirePackage{amssymb}
\RequirePackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

% utility macros
\newcommand{\alert}[1]{{\color{red}#1}\xspace}

% example boxes
\usepackage[most]{tcolorbox}
\newcounter{examplecounter}
\usepackage{xparse}
\def\exampletext{Example} % If English
\NewDocumentEnvironment{examplebox}{ O{} }
{
	\colorlet{titlecolor}{red!55!black} % Global example color
	\colorlet{bordercolor}{titlecolor} % Global example color
%	\colorlet{colexam}{blue!55!black} % Global example color
		
	\newtcolorbox[use counter=examplecounter]{myexamplebox}{%
		% Example Frame Start
		empty,% Empty previously set parameters
		title={\exampletext\ \thetcbcounter: #1},% use \thetcbcounter to access the testexample counter text
		% Attaching a box requires an overlay
		attach boxed title to top left,
		% Ensures proper line breaking in longer titles
		minipage boxed title,
		% (boxed title style requires an overlay)
		boxed title style={empty,size=minimal,toprule=0pt,top=0pt,bottom=3pt,left=3mm,overlay={}},
		coltitle=titlecolor,fonttitle=\sffamily,
		before=\par\medskip\noindent,parbox=false,boxsep=0pt,left=3mm,right=0mm,top=0pt,bottom=0pt,breakable,pad at break=0mm,
		before upper=\csname @totalleftmargin\endcsname0pt, % Use instead of parbox=true. This ensures parskip is inherited by box.
		% Handles box when it exists on one page only
		overlay unbroken={\draw[bordercolor,line width=.5pt] ([xshift=-0pt]title.north west) -- ([xshift=-0pt]frame.south west); },
		% Handles multipage box: first page
		overlay first={\draw[bordercolor,line width=.5pt] ([xshift=-0pt]title.north west) -- ([xshift=-0pt]frame.south west); },
		% Handles multipage box: middle page
		overlay middle={\draw[bordercolor,line width=.5pt] ([xshift=-0pt]frame.north west) -- ([xshift=-0pt]frame.south west); },
		% Handles multipage box: last page
		overlay last={\draw[bordercolor,line width=.5pt] ([xshift=-0pt]frame.north west) -- ([xshift=-0pt]frame.south west); },%
	}
	\begin{myexamplebox}}
	{\end{myexamplebox}\endlist
}

% vdots for non matrix usage
\makeatletter
\DeclareRobustCommand{\rvdots}{%
	\vbox{
		\baselineskip4\p@\lineskiplimit\z@
		\kern-\p@
		\hbox{.}\hbox{.}\hbox{.}
}}
\makeatother

% referencing description labels
%\RequirePackage{hyperref}
%\makeatletter
%\newcommand{\labitem}[2]{%
%	\def\@itemlabel{\textbf{#1}}
%	\item
%	\def\@currentlabel{#1}\label{#2}}
%\makeatother

% Theorem-style environments
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{thm}{Theorem}[section]
